On the Resilience of Routing Tables

Many modern network designs incorporate "failover" paths into routers' forwarding tables. We initiate the theoretical study of the conditions under which such resilient routing tables can guarantee delivery of packets.

==> positive.tex <==
%!TEX root = paper.tex

\section{Positive Result}

\begin{figure}[!ht]
  \begin{center}
\vspace{-10pt}
    \includegraphics[scale=0.2]{figure}
    \hspace{60pt}
    \includegraphics[scale=0.2]{negative_figure}
  \end{center}
%  \caption{Illustration}\label{fig:positive}
\vspace{-10pt}
\end{figure}

We now present our main result, which establishes that for every given network it is possible to efficiently compute a 1-resilient forwarding pattern.

\begin{thm}~\label{thm:t1fd}
For every network there exists a 1-resilient forwarding pattern and, moreover, such a forwarding pattern can be computed in polynomial time.
\end{thm}

We prove Theorem~\ref{thm:t1fd} constructively; we present an algorithm that efficiently computes a 1-resilient forwarding pattern. We now give an intuitive exposition of our algorithm (see~\cite{techrep} for a full proof). We first orient the edges in $G$ so as to compute a directed acyclic graph (DAG) $D$ in which each edge in $E$ is utilized. Our results hold regardless of how the DAG $D$ is computed. An example network and corresponding DAG appear in figures (a) and (b), respectively. The DAG $D$ naturally induces forwarding rules at source nodes; each node's incoming edge in $D$ is mapped to its first active outgoing edge in $D$, given some arbitrary order over the node's outgoing edges (\emph{e.g.}, node 4 in the figure forwards traffic from node 5 to node 2 if the edge to 2 is up, and to node 3 otherwise).
%Note that this does not yet fully specify the forwarding functions (as we have not yet specified to which edges nodes' outgoing edges in $D$ are mapped).

Intuitively, the next step is to identify a ``problematic'' node, that is, a node that is bi-connected to the destination in $G$ but not in the partial forwarding pattern computed thus far, and add forwarding rules so as to ``fix'' this situation. Once this is achieved, another problematic node is identified and fixed, and so on. Observe that nodes 1-4 in the figure are all problematic. Observe also that adding the two following forwarding rules fixes node 4 (\emph{i.e.}, makes node 4 bi-connected to the destination in the forwarding pattern): (a) when both of node 4's outgoing edges in $D$ are down, traffic reaching 4 from node 5 is sent back to 5; and (b) when node 5's direct edge to the destination is up, traffic reaching node 5 from node 4 is sent along this edge. Thus, the algorithm builds the forwarding functions at nodes gradually, as more and more forwarding rules are added to better the resilience of the forwarding pattern.

Implementing the above approach, though, requires care; the order in which problematic nodes are chosen, and the exact manner in which forwarding rules are fixed, are important. Intuitively, our algorithm goes over problematic nodes in the topological order $<_D$ induced by the DAG $D$ (visiting problematic nodes closer to the destination in $D$ first), and when fixing a problematic node $i$, forwarding rules are added until a minimal node in $<_D$ whose entire sub-DAG in $D$ does not traverse $i$ is reached. We prove that this scheme outputs the desired forwarding pattern in a computationally-efficient manner. 
